A Prediction-Correction Algorithm for Real-Time Model Predictive Control

In this work we adapt a prediction-correction algorithm for continuous time-varying convex optimization problems to solve dynamic programs arising from Model Predictive Control. In particular, the prediction step tracks the evolution of the optimal solution of the problem which depends on the current state of the system. The cost of said step is that of inverting one Hessian and it guarantees, under some conditions, that the iterate remains in the quadratic convergence region of the optimization problem at the next time step. These conditions imply (i) that the variation of the state in a control interval cannot be too large and that (ii) the solution computed in the previous time step needs to be sufficiently accurate. The latter can be guaranteed by running classic Newton iterations, which we term correction steps. Since this method exhibits quadratic convergence the number of iterations to achieve a desired accuracy $\eta$ is of order $\log_2\log_2 1/\eta$, where the cost of each iteration is approximately that of inverting a Hessian. This grants the prediction-correction control law low computational complexity. In addition, the solution achieved by the algorithm is such that the closed loop system remains stable, which allows extending the applicability of Model Predictive Control to systems with faster dynamics and less computational power. Numerical examples where we consider nonlinear systems support the theoretical conclusions.

==> intro_conf.tex <==
%!TEX root = root.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   A   B   S   T   R   A   C   T   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{abstract}
In this work, we consider the problem of Model Predictive Control (MPC). This approach to controlling dynamical systems requires the solution of a finite horizon dynamic program. Especially when the horizon is large, a limitation of this approach  is the computational burden.  This restricts the applicability of MPC to systems that have large time constants and/or high computational power since the solution needs to be computed in real time between control actions. To overcome these limitations, we propose a prediction-correction approach that allows computing an approximate solution of the MPC problem by performing exactly two Hessian inversions, i.e., with the same computational cost as performing two Newton steps. In addition, the stability guarantees of the closed-loop system are preserved. Numerical examples where we consider a highly nonlinear system support the theoretical conclusions.  
\end{abstract}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   S   E   C   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%


  \section{Introduction}
  Model Predictive Control is a control technique that selects the input of the system by solving a finite horizon optimization problem at each sampling time. The objective function one aims to minimize is related to the desired performance metric and the constraints represent the dynamics of the system and possible state and input constraints \cite{garcia1989model,qin2003survey}. The ability to impose these constraints is one of the main advantages of this method \cite{mayne2000constrained}. Its main drawback, however, is the computational cost associated to solving these optimization problems. In that sense, it is not surprising that MPC first found traction in the control of chemical processes \cite{allgower1999nonlinear,helbig1998model}%biegler1991optimization,
  , where the time constants are typically large and the systems are equipped with enough computational power. 

To overcome this limitations and to profit of the benefits of MPC in systems with fast dynamics and low computational power, on-line and efficient optimization methods are required. Several efforts based on Newton-type methods that aim to solve exactly the receding horizon problem, have been made \cite{li1989multistep,de1995extension}. However, if the time available for feedback is short, approximations are required. Some proposed algorithms consider a one step horizon in order to reduce the number of optimization variables \cite{choi1993feedback,choi1999instantaneous}. A common alternative is to perform linearizations of the system. This allows to solve the problem efficiently, because quadratic optimization problems with linear constraints can be solved with only one Newton step. Among these methods there are different approaches. Some linearize the system along a fixed optimal \cite{kramer1987numerical,kugelmann1990new,bock2000direct} or approximately optimal \cite{diehl2005real,diehl2005nominal}  trajectory over the whole time horizon. These solutions work well for nonlinear systems as long as the system is not largely disturbed and it stays close to the nominal solution. Another option is to directly linearize the dynamics of the system \cite{garcia1984quadratic,zheng1997computationally}. The performance of these methods relies on the system having small variation.

%Other possible linearization consist in performing successive linearizations along approximately optimal trajectories \cite{diehl2005real,diehl2005nominal} and linearization of the dynamics of the system \cite{garcia1984quadratic,zheng1997computationally}. 

In general, these methods do not exploit the fact that the different optimization problems that need to be solved are such that their optimal solution varies smoothly with the state of the system. This idea can be used to predict the solution of the problem in the next control interval based on the variation of the states. This idea has been exploited in the context of time-varying convex optimization to solve unconstrained \cite{simonetto2016class} and constrained \cite{ fazlyab2017prediction} problems efficiently. The general idea is to combine a prediction step that takes into account the temporal evolution of the optimization problem so that the predicted iterate does not drift away from the quadratic convergence neighborhood of the optimum, hence reducing the number of  Newton steps -- also named correction steps. {The prediction step is based on the implicit function theorem, and it has been used in \cite{zavala2009advanced} to solve the MPC problem approximately around a nominal state. } The computational cost of the aforementioned prediction is that of inverting a Hessian, which is the same as in Newton's method.

In \cite{paternain2018prediction} a prediction-correction algorithm to solve MPC was proposed which requires only one correction step, hence, with the same computational complexity as performing two Newton iterations. However, for the latter to hold, restrictive assumptions on the variation of the system between consecutive control intervals are imposed. In this work we relax these assumption by considering a multi-correction step (Section \ref{sec_algorithm}) and we establish a bound on the complexity of the algorithm based on the variation of the system (Section \ref{sec_convergence}). In Section \ref{sec_examples} we expand the numerical results of \cite{paternain2018prediction} to demonstrate the reduction in the computation of prediction-correction algorithms when compared to MPC. 


%
%\medskip\noindent{\bf Notation and definitions.} Let $\mathcal{M}^{n\times n}$ be the subspace of the $n \times n$ matrices. Let $\lambda_{\min}$ and $\lambda_{\max}$ be the eigenvalues of a matrix $A \in \mathcal{M}^{n \times n}$ with smallest and largest absolute values respectively. Then, the condition number of the matrix $A$ is the quotient $\lambda_{\max}/\lambda_{\min}$.

